The distribution of the length of the longest path in random acyclic orientations of a complete bipartite graph

Randomly sampling an acyclic orientation on the complete bipartite graph $K_{n,k}$ with parts of size $n$ and $k$, we investigate the length of the longest path. We provide a probability generating function for the distribution of the longest path length, and we use Analytic Combinatorics to perform asymptotic analysis of the probability distribution in the case of equal part sizes $n = k$ tending toward infinity. We show that the distribution is asymptotically Gaussian, and we obtain precise asymptotics for the mean and variance. These results address a question asked by Peter J. Cameron. Keywords: bipartite graph, directed graph, random graph, acyclic orientation, poly-Bernoulli numbers, lonesum matrices, generating function, analytic combinatorics, asymptotics.

==> bibliography.tex <==
\begin{thebibliography}{99}
 \addcontentsline{toc}{schapter}{\bibname}% This adds the Bibliography to the table of contents.
 \begin{spacing}{1} %This makes the bibliography single spaced.
\bibitem{B1}
G. Chartrand, L. Lesniak, and P. Zhang, {\it Graphs \& Digraphs, Fifth Edition.} Chapman \& Hall/CRC, 2011.

\bibitem{b6}
P. Erd\"{o}s and T Gallai, Graphs with prescribed degrees of vertices (Hungarian). {\it Matematikai Lapok} {\bf 11} (1960) 264-274.

\bibitem{b7}
D. R. Fulkerson, A. J. Hoffman, and M. H. McAndrew, Some properties of graphs with multiple edges. {\it Canadian Journal of Mathematics} {\bf 17} (1965) 166-177.

\bibitem{b8} 
S. L. Hakimi, On the realizability of a set of integers as degrees of the vertices of a graph. {\it Journal of the Society for Industrial and Applied Mathematics} {\bf 10} (1962) 496-506.

\bibitem{B2}
    L. Hansen and M. Schultz, A Degree Problem in 			Graph Theory. {\it Journal of Undergraduate 					Mathematics} {\bf 23} (1991) 45-53.  % This is an example of how to reference an article.

\bibitem{b9}
V. Havel, A remark on the existence of finite graphs (Czech.). {\it \v Casopis P\v{e}st. Mat.} {\bf 80} (1955) 477-480.

\bibitem{B3}
    M. Schultz and M. Watson, From Equi-Graphical Sets to Graphical Permutations. {\it Journal 		of Combinatorial Mathematics and Combinatorial 				Computing} {\bf 50} (2004) 33-46.

\bibitem{B4}
 A. Tripathi and S. Vijay, A note on a theorem of Erdos \& Gallai. {\it Discrete Mathematics} {\bf 265} (2003) 		417-420.
 
\bibitem{B5}
 M. Watson, From equi-graphical sets to graphical permutations: A problem of degrees in graphs. Masters thesis. University of Nevada, Las Vegas, 2002.

 \end{spacing}
\end{thebibliography}


==> test.tex <==
test
